Average-Case Lower Bounds and Satisfiability Algorithms for Small Threshold Circuits

$ \newcommand{\cclass}[1]{{\normalfont\textsf{##1}}} $We show average-case lower bounds for explicit Boolean functions against bounded-depth threshold circuits with a superlinear number of wires. We show that for each integer $d > 1$, there is a constant $\varepsilon_d > 0$ such that the Parity function on $n$ bits has correlation at most $n^{-\varepsilon_d}$ with depth-$d$ threshold circuits which have at most $n^{1+\varepsilon_d}$ wires, and the Generalized Andreev function on $n$ bits has correlation at most $\exp(-{n^{\varepsilon_d}})$ with depth-$d$ threshold circuits which have at most $n^{1+\varepsilon_d}$ wires. Previously, only worst-case lower bounds in this setting were known (Impagliazzo, Paturi, and Saks (SICOMP 1997)). We use our ideas to make progress on several related questions. We give satisfiability algorithms beating brute force search for depth-$d$ threshold circuits with a superlinear number of wires. These are the first such algorithms for depth greater than 2. We also show that Parity on $n$ bits cannot be computed by polynomial-size $\textsf{AC}^0$ circuits with $n^{o(1)}$ general threshold gates. Previously no lower bound for Parity in this setting could handle more than $\log(n)$ gates. This result also implies subexponential-time learning algorithms for $\textsf{AC}^0$ with $n^{o(1)}$ threshold gates under the uniform distribution. In addition, we give almost optimal bounds for the number of gates in a depth-$d$ threshold circuit computing Parity on average, and show average-case lower bounds for threshold formulas of any depth. Our techniques include adaptive random restrictions, anti-concentration and the structural theory of linear threshold functions, and bounded-read Chernoff bounds.

==> tocspecial.tex <==
%% tocspecial.tex 2018-04-17   ToC style file
%------------------------------------------------------------------
% Filename: tocspecial.cls
% 
% This documentclass is intended for typesetting articles for the
% 
% Theory of Computing.
% 
% See http://theoryofcomputing.org for further details.
%
% Version 0.1 Initial combination of banners from previous style files.
% ------------------------------------------------------------------
%
%% Special issue banners:

\newcommand{\motwani}{Special issue in honor of Rajeev Motwani}
\newcommand{\boolean}{Special issue: Analysis of Boolean Functions}
\newcommand{\approxrandomBC}{Special issue: APPROX-RANDOM 2012}
\newcommand{\approxrandomBD}{Special issue: APPROX-RANDOM 2013}
\newcommand{\approxrandomBE}{Special issue: APPROX-RANDOM 2014}
\newcommand{\approxrandomBF}{Special issue: APPROX-RANDOM 2015}
\newcommand{\cccBF}{Special issue: CCC 2015}
\newcommand{\cccBG}{Special issue: CCC 2016}
\newcommand{\cccBH}{Special issue: CCC 2017}
\newcommand{\itcsBD}{Special issue: ITCS 2013}
%% explanation: BC = 2012 BD = 2013 ... CA = 2020 CB = 2021 ...

